PANE: scalable and effective attributed network embedding

Given a graph G where each node is associated with a set of attributes, attributed network embedding (ANE) maps each node v in G to a compact vector Xv, which can be used in downstream machine learning tasks. Ideally, Xv should capture node v's affinity to each attribute, which considers not only v's own attribute associations, but also those of its connected nodes along edges in G. It is challenging to obtain high-utility embeddings that enable accurate predictions; scaling effective ANE computation to massive graphs pushes the difficulty of the problem to a whole new level. Existing solutions largely fail on such graphs, leading to prohibitive costs, low-quality embeddings, or both. This paper proposes PANE, an effective and scalable approach to ANE computation for massive graphs that achieves state-of-the-art result quality on multiple benchmark datasets. PANE obtains high scalability and effectiveness through 3 main algorithmic designs. First, it formulates the learning objective based on a novel random walk model for attributed networks. Second, PANE includes a highly efficient solver for the above optimization problem, whose key module is a carefully designed initialization of the embeddings, which drastically reduces the number of iterations required to converge. Finally, PANE utilizes multi-core CPUs through non-trivial parallelization of the above solver, which achieves scalability while retaining the high quality of the resulting embeddings. The performance of PANE depends upon the number of attributes in the input network. To handle large networks with numerous attributes, we further extend PANE to PANE++. Extensive experiments, comparing 10 existing approaches on 8 real datasets, demonstrate that PANE and PANE++ consistently outperform all existing methods in terms of result quality, while being orders of magnitude faster.

==> abstract.tex <==
% \begin{abstract}

Given a graph $G$ where each node is associated with a set of attributes, \textit{attributed network embedding} (\textit{ANE}) maps each node $v \in G$ to a compact vector $X_v$, which can be used in downstream machine learning tasks. Ideally, $X_v$ should capture node $v$'s \textit{affinity} to each attribute, which considers not only $v$'s own attribute associations, but also those of its connected nodes along edges in $G$. %The latter depends on the graph structure, meaning that the embeddings must incorporate the information of both node attributes and topological features of the graph. Hence, 
It is challenging to obtain high-utility embeddings that enable accurate predictions; scaling effective ANE computation to massive graphs with millions of nodes %(\textit{e.g.}, with millions of nodes and billions of edges)
%while retaining high result quality 
pushes the difficulty of the problem to a whole new level. Existing solutions largely fail on such graphs, leading to prohibitive costs, low-quality embeddings, or both.

%Given an attributed network $G =(V, R, E_V, E_R)$ consisting of a set $V$ of $n$ nodes, a set $R$ of $d$ attributes, a set $E_V$ of node-to-node edges and a set $E_R$ of node-attribute associations, {\em attributed network embedding} (ANE) aims to map each node $v \in V$ to a fixed-length embedding vector that captures both the attributes and topological features of $v$. 
%Although there exist several approaches to ANE that obtain effective embeddings, to our knowledge none of them scale to massive graphs with millions of nodes, due to the prohibitive cost of factorizing an $O(n^2)$-sized dense matrix, or training a deep neural network. In addition, most existing methods address undirected graphs, leading to suboptimal embeddings for directed graphs.

%Existing methods either explicitly construct and factorize an $n\times n$ dense matrix, or rely on expensive training courses of deep learning techniques, leading to prohibitively high costs. Additionally, prior work is only applicable for undirected graphs, resulting in unsatisfactory performance on directed graphs, where a node has two roles: source node and target node.

This paper proposes \algopt, an effective and scalable approach to ANE computation for massive graphs that achieves state-of-the-art result quality on multiple benchmark datasets, measured by the accuracy of three common prediction tasks: attribute inference, link prediction, and node classification. In particular, for the large {\em MAG} data with over 59 million nodes, 0.98 billion edges, and 2000 attributes, \algopt is the only known viable solution that obtains effective embeddings on a single server, within 12 hours.

%using 10 CPU cores, 1TB memory, and 12 hours running time.
%; the resulting embeddings achieve over 0.88 average precision for attribute inference. 

\algopt obtains high scalability and effectiveness through three main algorithmic designs. First, it formulates the learning objective based on a novel random walk model for attributed networks.
%, which effectively captures node-attribute affinity over multiple hops. 
The resulting optimization task is still challenging on large graphs. %, as it involves the joint factorization of two large matrices. 
Second, \algopt includes a highly efficient solver for the above optimization problem, whose key module is a carefully designed initialization of the embeddings, which drastically reduces the number of iterations required to converge. Finally, \algopt utilizes multi-core CPUs through non-trivial parallelization of the above solver, which achieves scalability while retaining the high quality of the resulting embeddings. Extensive experiments, comparing 10 existing approaches on 8 real datasets, demonstrate that \algopt consistently outperforms all existing methods in terms of result quality, while being orders of magnitude faster.

%generates higher quality embeddings compared to all existing methods, at a fraction of their computational cost.

%effective embeddings with superior results f (i) the embeddings generated by \algopt lead to superior results for three common tasks: attribute inference, link prediction, and node classification, and (ii) the computation overhead of \algopt is orders of magnitude smaller than competing methods. 


%novel ANE solution that is capable of obtaining high-quality node and attribute embeddings for large (directed or undirected) graphs with millions of nodes. In particular, the effectiveness of \algopt is obtained through a construction of node-attribute co-embeddings guided by their pointwise mutual information (PMI) over multiple hops, while the efficiency of \algopt is achieved through a carefully designed algorithm that reduces the embedding construction to a joint factorization of two size-$O(n \cdot d)$ matrices, where $n$ is the number of nodes and $d$ is the number of attributes. 
%algorithm that only factorizes a size-$O(n \cdot d)$ matrix instead of an $O(n^2)$-sized one
%. Going one step further, 
%In addition, we present a non-trivial parallel version \algoptp that utilizes modern multi-core processors to accelerate ANE computation, without compromising the result quality. 

%Extensive experiments on 8 real datasets against 10 existing approaches demonstrate that (i) the embeddings generated by \algopt lead to superior results for three common tasks: attribute inference, link prediction, and node classification, and (ii) the computation overhead of \algopt is orders of magnitude smaller than competing methods. 

%Furthermore, when using 10 threads, \algoptp accelerates \algopt by up to 9 times, and is able to process an attributed network with 59.3 million nodes, 0.98 billion edges, and 2000 attributes within $12$ hours.


%This paper studies \textit{attributed directed network co-embedding}, which aims to learn a source-node embedding vector, a target-node embedding vector for each node, and an attribute embedding vector for each attribute, such that not only node-node associations but also node-attribute associations are effectively captured. 

%Our proposed solution, , is built on the novel idea of deriving high-quality embedding vectors by jointly factorizing {\em forward SPMI} and {\em backward SPMI} matrices, which quantify the high-order node-attribute associations when the nodes play the roles of source nodes and target nodes, \eg followers and followees in social networks, respectively. 

%\algoptp further improves \algopt with non-trivial parallel techniques geared towards for higher efficiency without compromising effectiveness.



% \end{abstract}

